A General Algorithm for Solving Rank-one Matrix Sensing

Matrix sensing has many real-world applications in science and engineering, such as system control, distance embedding, and computer vision. The goal of matrix sensing is to recover a matrix $A_\star \in \mathbb{R}^{n \times n}$, based on a sequence of measurements $(u_i,b_i) \in \mathbb{R}^{n} \times \mathbb{R}$ such that $u_i^\top A_\star u_i = b_i$. Previous work [ZJD15] focused on the scenario where matrix $A_{\star}$ has a small rank, e.g. rank-$k$. Their analysis heavily relies on the RIP assumption, making it unclear how to generalize to high-rank matrices. In this paper, we relax that rank-$k$ assumption and solve a much more general matrix sensing problem. Given an accuracy parameter $\delta \in (0,1)$, we can compute $A \in \mathbb{R}^{n \times n}$ in $\widetilde{O}(m^{3/2} n^2 \delta^{-1} )$, such that $ |u_i^\top A u_i - b_i| \leq \delta$ for all $i \in [m]$. We design an efficient algorithm with provable convergence guarantees using stochastic gradient descent for this problem.

==> conclusion.tex <==


\section{Conclusion}\label{sec:conclusion}
In this paper, we study the problem of matrix sensing which has a wide variety of practical applications in real-world science and engineering problems like image processing, quantum computing, and sensor localization. In many application domains of matrix sensing, it is appealing to tradeoff accuracy for fast running time, e.g., in fast and approximated $k$-nearest neighbors and $k$-means.
We design an efficient algorithm with provable convergence guarantees using stochastic gradient descent to approximate matrix sensing.
 
